MemexQA: Visual Memex Question Answering

This paper proposes a new task, MemexQA: given a collection of photos or videos from a user, the goal is to automatically answer questions that help users recover their memory about events captured in the collection. Towards solving the task, we 1) present the MemexQA dataset, a large, realistic multimodal dataset consisting of real personal photos and crowd-sourced questions/answers, 2) propose MemexNet, a unified, end-to-end trainable network architecture for image, text and video question answering. Experimental results on the MemexQA dataset demonstrate that MemexNet outperforms strong baselines and yields the state-of-the-art on this novel and challenging task. The promising results on TextQA and VideoQA suggest MemexNet's efficacy and scalability across various QA tasks.

==> tex/_intro3.tex <==
\section{Introduction}
\label{sec:intro}

A typical smartphone user may take hundreds of photos when on vacation or attending an event. Within only a few years, one ends up accumulating dozens of thousands of photos and many hours of video, that capture cherishable moments from one's past. 
A recent study~\cite{jiang17delving} hints that people utilize personal photos as a mean of recovering pieces from their memories. 
% Manually searching through such large collections, however, still remains a daunting task. 
In this paper, we propose \textit{MemexQA}\footnote{\textit{Memex} was first posited by Bush in 1945~\cite{bush1945atlantic} as an enlarged intimate supplement to an individual's memory.}, a new AI task for question answering: given a collection of photos or videos from a user, the goal is to automatically answer questions that help recover his/her memory about the event captured in the collection. With conversational bots like Siri and Alexa becoming ubiquitous, natural language questions seem to be the best way of going down memory lane. A system utilizing MemexQA can be regarded as a personal assistant of one's past memories and can answer questions like ``Where did we last see fireworks?'' or `` Who had a birthday party in January 2017?'', as long as media that contain the answer exist in our collection.

In order to derive an answer for such questions, we rely not only on visual understanding of single photos or videos, but the photo collection as a whole and select the corresponding photos and videos that may support the answers. 
To tackle this problem, we crowdsourced questions and answers for a large set of images~\cite{huang2016visual}, organized in user albums. The \textit{MemexQA dataset}
%\footnote{For the rest of the paper, we will refer to the MemexQA task as simply \textit{MemexQA} and to the proposed dataset as \textit{the MemexQA dataset} to clearly distinguish the two.} 
consists of 20,591 personal photos from 602 albums and 101 Flickr users.
Examples of questions, answers and photos from the dataset are illustrated in  Fig.~\ref{fig:intuition}.
% \yannis{should we maybe blur children's faces in the figs?}. 
The MemexQA dataset focuses on the four types of questions (what, who, when, and where) that are suggested by a recent study~\cite{jiang17delving} to cover a high percentage of personal photo annotations and queries. 



\begin{figure}[t!]
\centering
\vspace{-3mm}
\includegraphics[width=0.75\linewidth, height = 50mm]{figures/intuition}
\caption{\label{fig:intuition}Example MemexQA questions. The top panel displays sampled personal photos of a Flickr users, where each photo collage corresponds to an album. The bottom panel shows representative questions and answers about the photos. 
%Note that the MemexQA answers come from multimodal information about the photo content, timestamp, GPS, and album.
}
\vspace{-3mm}
\end{figure}

To illustrate the technical challenges in depth, it is helpful to discuss the difference between MemexQA and Visual QA (VQA)~\cite{antol2015vqa}. A hot research topic in recent years, VQA
% MemexQA presents differences Visual QA (VQA)~\cite{antol2015vqa}, which
is designed to answer natural language questions for an image, questions that a toddler or an alien would have trouble answering. 
%  such as ``what books are under the television'' or ``what is the color of the boat''. 
MemexQA also answers questions based on images, the questions however may possibly require reasoning over multiple images. The answers for MemexQA are not trivial even for an adult to answer manually, as it would require going through a large amount of media first.
We argue that MemexQA is more challenging than VQA in the following aspects:
 \vspace{-7pt}
\begin{description}
\setlength\itemsep{-2pt}
\item [Cross-media reasoning] MemexQA adds a localization component across media documents. One needs to inspect multiple items to find clues for the media that support the answer to a given question, while also properly understanding the (visual or otherwise) content of each document.
\item [Cross-modality reasoning] MemexQA utilizes multimodal knowledge to provide an answer, which may come from the visual content, incomplete captions, timestamps or GPS. It therefore requires some form of reasoning across multimodal information from a large scale dataset. Of course this extended to any extra annotations that a collection might have, \emph{e.g.} face/person identification, action recognition, depth.
 \item [Dynamic answer space / memory] The answer space for MemexQA is somewhere between the closed set of most current VQA tasks and open-ended QA, as it is conditioned on the database. However, not only this space is not predefined and different among users, it also grows as the database increases. This is far larger than any current VQA task. Furthermore, MemexQA has an information retrieval component and takes into account the evergrowing dynamic memory of a user's media collection. This implicitly connects the task to personalization as the same question would give totally different answers for 2 different users.
\end{description}

\alert{We believe that MemexQA is a highly applicable task that is not a proxy, like VQA, tries to solve a problem for which is searching our personal media collections. According to our experiments, users spend 10x longer in answering a MemexQA than a VAQ question.}
% \lu{help user more than VQA. According to our experiments, users spend 10x longer in answering a MemexQA than a VAQ question.}


In this paper we further present a novel approach towards solving the MemexQA task. We propose\textit{MemexNet}, an united network architecture for image, text and video question answering. Motivated by the Watson QA system~\cite{ferrucci2010building} we build three major modules in MemexNet: the question understanding network, search engine, and answer inference module. Our approach consists of end-to-end trainable networks learned together with off-the-shelf image/video engines, while utilizing residual connections from the question understanding to the answer inference module.
To summarize, are contributions are the following:
\begin{itemize}
\setlength\itemsep{-2pt}
\vspace{-3mm}
\item We introduce a new task, MemexQA, as well as a large, croudsourced dataset that consists of question and answer pairs corresponding to not just single images but also sets of images.
\item We propose a novel approach to tackle MemexQA via a unified, end-to-end trainable model that encompasses query understanding, large-scale search and answer inference module.
\item We present extensive experimental results on the MemexQA dataset and demonstrate that the proposed method outperforms all strong baselines and yields the state-of-the-art on a very challenging dataset. We further compare MemexNet against recent approaches for text and video QA on popular public datasets and demonstrate competitive results in all QA tasks.
\end{itemize}


\vspace{-3mm}
We consider MemexQA to be a multi-disciplinary research task as it combines computer vision, natural language processing and large-scale information retrieval. We believe that this combination will enable us to scale MemexQA to real-world applications and the rapidly growing user media collections.

\lu{ To the best of our knowledge, it is the first attempt to tackle the large-scale video QA problem.}


(the following are to be revised) In summary, MemexNet is characterized by three features:

\begin{itemize}
\vspace{-3mm}
\item End-to-end trainable networks learned together with off-the-shelf image/video engines.
\vspace{-1mm}
\item Residual connections from the question understanding to the answer inference module.
\vspace{-1mm}
\item Configurable modular neural networks for answer inference.
\vspace{-3mm}
\end{itemize}



==> tex/intro.tex <==
\section{Introduction}
\label{sec:intro}

%1) Explain the selling points clearly in the Introduction;
%2) technical difference with TextQA, VQA. Use a picture to illustrate the difference

%\yannis{For me, the biggest difference from generic VQA is the Memex: we have a "memory" in the pipeline, we answer questions given a collection, on the collection itself. So unlike VQA that tries to answer questions for new images, our goal is to answer questions *given* the users images. VQA is still part of our picture, but we go a step further, and our answers conditioned on the collection and the video content engine results, while we might use multiple images to answer the question. it is a form of "Conditional VQA". The pipeline is clear from Fig~\ref{fig:framework}, but we can have another fig that also puts traditional VQA in the picture. Can try making it.}



The prevailing of mobile devices and cloud services has led to an unprecedented growth of personal photos and videos~\citet{googlephoto}. These photos capture cherishable moments in our lives, e.g. wedding ceremonies, vacations, birthday parties, baby showers, graduation ceremonies, etc., and thus carry great sentimental value for their owners. 
A recent study on personal media search~\citet{jiang17delving} suggests people utilize personal photos as a way of recovering pieces from their memories, e.g. looking for a specific name, place or date usually in the question format, e.g. ``where did we go last Christmas?'', or ``how many times did we have pizza last week?''. Due to the large quantity and lack of textual metadata, manually answering questions within personal photos is a cumbersome and prolonged task.

Deep learning has enabled automatic QA (Question Answering) by both vision and language. A representative task is VQA (Visual QA), where given an image, the goal is to answer questions about the image that a toddler or an alien would have trouble answering~\citet{antol2015vqa}. 
A multitude of approaches have been recently proposed in the VQA framework and have shown notable progress in terms of performance on public benchmark datasets~\citet{zhu2016visual7w, NamHK16}.
% However, these VQA solutions may not be used to answer questions about personal photos for the following reasons. First, the answer about personal photos is usually recovered across multiple photos as opposed to from a single image. Indeed, we need to examine lots of, and in many cases all, personal photos to answer a simple question like ``how many times did we have pizza?''. Second, VQA relies only on the photo content to answer a question. In reality, however, many types of questions, such as when and where questions, need extra information about the photo such as the photo's timestamp, GPS (if any), and   album information. The insufficient information significantly limits the diversity of VQA questions. For example, to answer the question ``where did we last see the fireworks?'', not only do we need visual object fireworks, but also GPS information and timestamps to find the location and latest photos. Due to the limitations, VQA is an interesting but arguably less practically useful task.
However, such VQA approaches are not really suited for answering meaningful questions on personal collections. First, in many cases the answer may come not from a single photo in the collection, but has to be recovered \textit{across multiple photos}. Indeed, we need to examine lots of, and in many cases all, personal photos to answer a simple question like ``how many times did we have pizza last year?''. Secondly, VQA relies only on the photo's visual content to answer a question. Many types of questions, though, such as when and where questions, require extra information about the photo, like the photo's timestamp, location (if any) and album information. The absence of other metadata significantly limits the diversity of VQA questions. For example, to answer the question ``where did we last see fireworks?'', not only do we need to be able to visually detect fireworks, but we also need GPS information and timestamps to find the location and latest photos. Although undoubtedly a very important step towards scene perception, VQA is arguably less practical and useful as a task.

\begin{figure}[t!]
\centering≥
\vspace{-3mm}
\includegraphics[width=0.8\linewidth]{figures/intuition}
\caption{\label{fig:intuition}Example MemexQA questions collected via Amazon Mechanical Turk. The top panel shows the question and answer~\yannis{will it?}. The bottom panel displays selected personal photos, where each row is an album. Note that the MemexQA answers come from multiple photo content, timestamp, GPS, and album information.}
\vspace{-3mm}
\end{figure}

In this paper, we propose a new task for query answering we call MemexQA (Memex QA), which is defined as: Given a collection of photos or videos from a user, the goal is to automatically answer questions that help recover his/her memory about an event captured in the collection. Fig.~\ref{fig:intuition} illustrates representative MemexQA questions for a real Flickr user~\yannis{let's not push it on how these come from real users... sounds bad to me}, where the top panel shows representative MemexQA questions/answers, and the bottom panel displays selected personal photos organized in 4 albums. The name MemexQA is inspired by the fictional device called Memex posited by Bush in 1945~\citet{bush1945atlantic}, which he presented as an enlarged intimate supplement to an individual's memory. MemexQA is an embodiment of Memex to analyze one's personal photos or videos so that it may be later consulted with exceeding speed and flexibility. In this perspective, MemexQA can be regarded as a personal assistant of one's past memories. 

According to~\citet{antol2015vqa}, MemexQA is a compelling AI (Artificial Intelligence) task as it (i) requires multimodal knowledge beyond a single domain and (ii) has a well-defined quantitative evaluation metric. More importantly, MemexQA is a very useful functionality to tackle the real-world challenge of searching information in a large amount of personal photo or video collection~\citet{garrigues2016tag,jiang17delving}. In summary, MemexQA has several key differences with existing VQA: 1) MemexQA introduces a notion of cross-image QA, where a question can be answered by considering a collection of photos. 2) the goal of MemexQA is to facilitate ``real users'' rather than ``toddlers'' in VQA. Given an image, it is trivial for an adult to answer a VQA question within a few second. However, it is considerably more difficult, and might take minutes for the same adult to answer a MemexQA question. The data analysis in Section~\ref{tab:dataset_comp} substantiates this claim. Therefore, MemexQA may help real users consult his memory with exceeding speed and flexibility. 3) MemexQA utilizes multimodal information, including vision, language, and metadata, to answer a question. Indeed, visual information is the most important modality as xxxxxx. More diverse questions can be answered by combining metadata and language, e.g. ``when did I last see the fireworks near the magic castle in Orlando?''
% a more realistic dataset?

We present a first-of-its-kind dataset on MemexQA, which contains 13,591 personal photos from 101 real Flickr users. For each photo, We collect a variety types of multimodal information including, the timestamp, title, tags, GPS (if any), album information, and captions. The dataset contains 8,876 questions and 177,520 multiple choice answers\footnote{We are collecting a larger dataset for 1.0 version}. For each question, the annotator also provides evidential photos to justify their answers, and there are totally 14,680 evidential photos. Motivated by Flickr top query terms, we focus on the following type of questions: what ()
To reduce the ambiguous and low-quality QA, each photo is annotated by at least 2 workers and verified by 3 workers, independently. Note that the sheer amount of that MemexQA is smaller than that of the VQA dataset. To address the MemexQA problem, this paper also introduces a novel neural network method. Essentially it consists of three major components: a recurrent neural network to understand the question, a content-based engine to analyze and find relevant videos, and a multi-channel attention neural network to extract the answer. The model can be trained in an end-to-end fashion. Experimental results on MemexQA dataset demonstrates the proposed method outforms baseline methods and achieve the state-of-the-art result on the dataset.

MemexQA is a multi-disciplinary AI research problem. which combines Computer Vision, natural language processing, and information retrieval. MemexQA advances VQA in . It allows for a better marriage between language and vision in solving a real-word important problem. We envision MemexQA to contribute to a 



\lu{privacy smaller data}



==> tex/intro2.tex <==
\section{Introduction}
\label{sec:intro}

% structure
% 1. motivation
% 2. what is memex QA (with some key modules)
% 3. differences with VQA
%	(a) classification -> search
%	(b) align photos, meta data
%	(c) scale ? what is the number of videos
% summarize: VQA aims to pass Turning test, but Memex QA is to be faster and more efficient than human. 
% Despite its effectivenss, Turing test may not be passed in the short time, while Memem QA could assistant anyone with their flooding media data  
%
% 4. technical challenges

Consider a scenario of searching through personal photos and videos: a typical smartphone user may shoot hundreds of photos when taking a tour or attending an event, and accumulate dozens of thousands of photos in only a few years. In addition, 
the user likely further captures many hours of videos every year.
% the user likely captures a lot of videos with hundreds of megabytes. 
What can the user do with these photos and videos?
A recent study~\citet{jiang17delving} suggests that people utilize personal photos as a way of recovering pieces from their memories,
e.g. ``where did we go last Christmas?'', or ``how many times did we have pizza last week?''. To find the answer, most likely it will take a long time for the user  to browse his/her photo collections. 


In this paper, we propose MemexQA\footnote{The name \textit{Memex} comes from the fictional device posited by Vannevar Bush in his visionary article pumlished in 1945~\citet{bush1945atlantic}, which the author presented as an enlarged intimate supplement to an individual's memory.}, a new task for query answering: given a collection of photos or videos from a user, the goal is to automatically answer questions that help recover his/her memory about an event captured in the collection. 
MemexQA can be regarded as a personal assistant of one's past memories by answering questions like ``Where did we last see fireworks'', or `` Who had a birthday party in January 2017''? 
In order to retrieve the right answer for such questions, we rely not only on visual understanding, but we also need to examine the user's collection as a whole and select the corresponding photos and videos which support the answers. 

To tackle this problem, we crowdsourced  questions and answers for a large set of images from SIND dataset~\citet{huang2016visual}, organized in user albums. The \textit{MemexQA dataset}\footnote{For the rest of the paper, we will refer to the MemexQA task as simply \textit{MemexQA} and to the proposed dataset as \textit{the MemexQA dataset} to clearly distingush the two.} consists of 13,591 personal photos from 602 albums and 101 Flickr users. Examples of questions, answers and photos from the dataset are illustrated in  Fig.~\ref{fig:intuition}. The MemexQA dataset focuses on four types of questions: what, who, when, and where. These 4W questions are suggested by a recent study~\citet{jiang17delving} to cover a high percentage of personal photo annotations and queries. 


\begin{figure}[t!]
\centering
\vspace{-3mm}
\includegraphics[width=0.9\linewidth, height = 60mm]{figures/intuition}
\caption{\label{fig:intuition}Example MemexQA questions collected via Amazon Mechanical Turk. The top panel displays personal photos of a Flickr users, where each photo collage corresponds to an album. The bottom panel shows representative MemexQA questions/answers. Note that the MemexQA answers come from multimodal information about the photo content, timestamp, GPS, and album. }
\vspace{-3mm}
\end{figure}



To illustrate the technical challenges in depth, it is helpful to discuss the difference between MemexQA and recent works on Visual QA (VQA)~\citet{antol2015vqa}. A hot research topic in recent years, VQA is designed to answer natural language questions for an image, questions that a toddler or an alien would have trouble answering. 
%  such as ``what books are under the television'' or ``what is the color of the boat''. 
MemexQA also answers questions based on images, but the questions are possibly targeting not just one image, but an album or the whole collection of a user's photos. What is more, the answers for MemexQA are not trivial even for an adult to answer, as it would require going through a large amount of media.

We argue that MemexQA is more challenging task than VQA in the following aspects:
 \vspace{-7pt}
\begin{description}
\setlength\itemsep{-2pt}
 \item [Cross-media reasoning] MemexQA adds a localization component across media documents. One needs to inspect multiple items to find clues for the media that support the answer to a given question, while also properly understanding the (visual or otherwise) content of each document.
 \item [Cross-modality reasoning] MemexQA utilizes multimodal knowledge to provide an answer, which may come from the visual content, incomplete captions, timestamps or GPS. It therefore requires some form of reasoning across multimodal information from a large scale dataset. Of course this extended to any extra annotations that a collection might have, \emph{e.g.} face/person identification, action recognition, depth.
 \item [Dynamic answer space / memory] The answer space for MemexQA is somewhere between the closed set of most current VQA tasks and open-ended QA, as it is conditioned on the database. However, not only this space is not predefined and different among users, it also grows as the database increases. This is far larger than any current VQA task.
 \item [Towards personalized answers] MemexQA has an information retrieval component and takes into account the evergrowing dynamic memory of a user's media collection. This implicitly connects the task to personalization as the same question would give totally different answers for 2 different users.
 \end{description}

\alert{
\begin{description}
\setlength\itemsep{-2pt}
 \item [Beyond classification] In many recent papers, VQA is solved as a classification problem. The output of the VQA classifier is the confidence over a list of given answers. In contrast, MemexQA requires to find the clues from personal photo collections, and locate the images related to the given question. To this goal, we have to build a new model to solve the localizing problem. 
 \item [Aligning multiple images and meta data] MemexQA utilizes multimodal knowledge include visual, incomplete captions, and GPS. One challenge lies in how to align large scale multi-modal information into the same semantic space. This is more challenging than captioning a single image as in VQA.
 \item [Scale] MemexQA provides a very useful tool to tackle the real-world challenge of searching information in a large amount of personal photo or video collection. \llc{Lu: pls fill in the size of video dataset?} \yannis{I dont think we need to talk about our dataset at all in this part; we are pitching the task here, no?}
 \end{description}
}

\alert{
We believe that MemexQA is a very interesting and highly applicable task that tries to solve the important problem which is searching our personal media collections. We are potentially dealing with personal, cherishable moments in a person's life, e.g. wedding ceremonies, vacations, birthday parties, graduation ceremonies, etc., and such collections carry great sentimental value for their owners.
}

% Note the first study this paper does not aim to answer to any possible question as in VQA. The major goal of MemexQA is to help real users consult their memory with exceeding speed and flexibility. 
% \yannis{this whole paragraph can go to the dataset section}


% limitation of VQA:
%for which the question words usually have dominant influence on predicting the answer. For example, the correctly predicted answers for the two questions given for the first image ‘what is the color of sofa’ and ‘which brand is the laptop’come mostly from the question words, without the need for image. This demonstrates the bias in the frequency of object and actions appearing in the images of COCO dataset.

\alert{
% In this paper we define MemexQA, present a crowdsourced dataset and propose an end-to-end model for solving the task.
Given the complexity of the task, we have to go beyond both VQA and TextQA to give proper answers: We utilize cross-dimensional attention mechanisms on both the images of the collection and the multiple modalities for each image. Indeed, our model outperforms all strong baselines on the task. To summarize, our contributions are the following:
\begin{itemize}
\setlength\itemsep{-2pt}
\item We introduce a new task, MemexQA, as well as a large, croudsourced dataset that consists of question and answer pairs corresponding to not just specific images but also \textit{user image collections}.
\item We propose a novel approach to tackle MemexQA and present \textit{MemexNet}, a unified, end-to-end trainable model that encompasses query understanding, large-scale search and multi-modal attention components.
\item We present extensive experimental results on the MemexQA dataset and demonstrate that the proposed method outperforms all strong baseline methods and yields the state-of-the-art on a very challenging dataset.
\end{itemize}


MemexNet has three key components/modules: Question understanding, large scale content search engine, multi-channel attention/clue localization. Some components are not novel in isolation, \emph{e.g.} the question understanding model is borrowed from NLP~\citet{?}. However, MemexNet as a whole possesses novelty: the memory/collection search engine is a generalization of~\citet{elamp} for multi-modal data, the multi-channel attention across modalities is ??\yannis{Lu, can you fill in sth here - I am unsure about the details...}, while the whole model can be trained in an end-to-end fashion. 

We consider MemexQA to be a multi-disciplinary AI research task as it combines computer vision, natural language processing and large-scale information retrieval. We believe that this combination will enable us to scale MemexQA to real-world applications and the rapidly growing user media collections.
}


% To address the MemexQA problem, this paper proposes  a novel model with three key components:
% \begin{itemize}
% \item Question understanding (to be filled in)
% \item Large scale content search engine(to be filled in)
% \item Multi-channel attention/clue localization (to be filled in)
% \end{itemize}
% To facilitate the large scale learning, we build a unified model named ``MemexNet''which can be trained in an end-to-end fashion. Experimental results on MemexQA dataset demonstrates the proposed method outforms baseline methods and achieve the state-of-the-art result on the dataset\llc{can we use stronger claim here?}.


%According to~\citet{antol2015vqa}, MemexQA is a compelling AI (Artificial Intelligence) task as it (i) requires multimodal knowledge beyond a single domain and (ii) has a well-defined quantitative evaluation metric. More importantly, MemexQA is a very useful functionality to tackle the real-world challenge of searching information in a large amount of personal photo or video collection~\citet{garrigues2016tag,jiang17delving}. In summary, MemexQA has several key differences with existing VQA: 1) MemexQA introduces a notion of cross-image QA, where a question can be answered by considering a collection of photos. 2) the goal of MemexQA is to facilitate ``real users'' rather than ``toddlers'' in VQA. Given an image, it is trivial for an adult to answer a VQA question within a few second. However, it is considerably more difficult, and might take minutes for the same adult to answer a MemexQA question. The data analysis in Section~\ref{tab:dataset_comp} substantiates this claim. Therefore, MemexQA may help real users consult his memory with exceeding speed and flexibility. 3) MemexQA utilizes multimodal information, including vision, language, and metadata, to answer a question. Indeed, visual information is the most important modality as xxxxxx. More diverse questions can be answered by combining metadata and language, e.g. ``when did I last see the fireworks near the magic castle in Orlando?''

%The prevailing of mobile devices and cloud services has led to an unprecedented growth of personal photos and videos~\citet{googlephoto}. These photos capture cherishable moments in our lives, e.g. wedding ceremonies, vacations, birthday parties, baby showers, graduation ceremonies, etc., and thus carry great sentimental value for their owners. 
 %e.g. looking for a specific name, place or date usually in the question format, 
%Due to the large quantity and lack of textual metadata, manually answering questions within personal photos is a cumbersome and prolonged task.

%illustrates representative MemexQA questions  
%for a real Flickr user~\yannis{let's not push it on how these come from real users... sounds bad to me}, 
%where the top panel shows representative MemexQA questions/answers, and the bottom panel displays selected personal photos organized in 4 albums.  MemexQA is an embodiment of Memex to analyze one's personal photos or videos so that it may be later consulted with exceeding speed and flexibility. 



